Traced monoidal categories as algebraic structures in $\mathbf{Prof}$

We define a traced pseudomonoid as a pseudomonoid in a monoidal bicategory equipped with extra structure, giving a new characterisation of Cauchy complete traced monoidal categories as algebraic structures in $\mathbf{Prof}$, the monoidal bicategory of profunctors. This enables reasoning about the trace using the graphical calculus for monoidal bicategories, which we illustrate in detail. We apply our techniques to study traced $*$-autonomous categories, proving a new equivalence result between the left $\otimes$-trace and the right $\unicode{8523}$-trace, and describing a new condition under which traced $*$-autonomous categories become autonomous.

==> main-dot2tex-fig1.tex <==

\begin{tikzpicture}[line join=bevel,]
%%
\node (0) at (30.0bp,340.5bp) [] {
    \begin{tikzpicture}[baseline=(current bounding box.center)]
      \node[comult] (c) {};
      \node[twfrobcap, anchor=rightleg] (cap) at (c.leftleg) {};
      \node[comult, dot=black, anchor=rightleg, span=1.5] (c') at (c.bottom) {};
      \idstack[anchor=cap.leftleg]{1}
      \idstack[anchor=c.rightleg, direction=up]{2}
      \node[comult, dot=black, anchor=rightleg] (c'') at (c'.bottom) {};
      \node[comult, anchor=bottom] (c''') at (id2.top) {};
      \node[twfrobcap, anchor=rightleg, span=1.75] (cap') at (c'''.leftleg) {};
      \draw (cap'.leftleg) -- (c''.leftleg);
      \idstack[anchor=c'''.rightleg, direction=up]{2}
      \node[draw=blue, dashed, fit={(c''.bottom) (c''.leftleg) (c'.rightleg)}]{};
      \node[draw=blue, dashed, fit={(c.bottom) (c.leftleg) (c'''.rightleg)}]{};
      \node[draw=red, dashed, fit={(c.rightleg) (c'.south) (cap.top) (cap.leftleg)}]{};
    \end{tikzpicture}
    };
  \node (1) at (502.5bp,422.5bp) [] {
    \begin{tikzpicture}[baseline=(current bounding box.center)]
      \node[comult] (c) {};
      \node[twfrobcap, anchor=rightleg] (cap) at (c.leftleg) {};
      \node[comult, dot=black, anchor=rightleg, span=1.5] (c') at (c.bottom) {};
      \idstack[anchor=cap.leftleg]{1}
      \idstack[anchor=c.rightleg, direction=up]{2}
    \end{tikzpicture}
    };
  \node (3) at (171.0bp,340.5bp) [] {
    \begin{tikzpicture}[baseline=(current bounding box.center)]
      \node[mult] (m) {};
      \node[mult, dot=black, anchor=leftleg, span=1.5] (m') at (m.top) {};
      \node[twfrobcup, anchor=leftleg] (cup) at (m.rightleg) {};
      \node[identity, anchor=top] at (m'.rightleg) {};
      \idstack[anchor=m.leftleg]{1}
      \node[twfrobcup, anchor=rightleg] (cup') at (id1.bottom) {};
      \node[twfrobcap, anchor=leftleg] (cap) at (m'.top) {};
      \idstack[anchor=cap.rightleg]{5}
      \node[comult, dot=black, anchor=rightleg, span=4.75] (c) at (id5.bottom) {};
      \idstack[anchor=cup'.leftleg, direction=up]{3}
      \node[comult, anchor=bottom] (c') at (id3.top) {};
      \node[twfrobcap, anchor=rightleg] (cap') at (c'.leftleg) {};
      \draw (cap'.leftleg) -- (c.leftleg);
      \idstack[anchor=c'.rightleg, direction=up]{2}
      \node[draw=red, dashed, fit={(m'.top) (m.leftleg) (cup.bottom) (m'.rightleg)}]{};
    \end{tikzpicture}
    };
  \node (12) at (171.0bp,154.5bp) [] {
    \begin{tikzpicture}[baseline=(current bounding box.center)]
      \node[comult, dot=black, span=2.5] (c) {};
      \node[comult, dot=black, anchor=bottom] (c') at (c.leftleg) {};
      \node[comult, anchor=bottom] (c'') at (c.rightleg) {};
      \node[comult, anchor=bottom] (c''') at (c''.leftleg) {};
      \node[twfrobcap, anchor=rightleg] (cap) at (c'''.leftleg) {};
      \node[identity, anchor=bottom] (i) at (c'''.rightleg) {};
      \node[swishr, anchor=bottom] (s) at (i.top) {};
      \node[twfrobcap, anchor=rightleg, span=2] (cap') at (s.top) {};
      \draw (cap.leftleg) -- (c'.rightleg);
      \draw (cap'.leftleg) -- (c'.leftleg);
      \idstack[anchor=c''.rightleg, direction=up]{5}
    \end{tikzpicture}
    };
  \node (2) at (1056.5bp,410.5bp) [] {
    \begin{tikzpicture}[baseline=(current bounding box.center)]
      \idstack{3}
    \end{tikzpicture}
    };
  \node (5) at (663.0bp,361.5bp) [] {
    \begin{tikzpicture}[baseline=(current bounding box.center)]
      \node[mult] (m) {};
      \node[mult, dot=black, anchor=leftleg, span=1.5] (m') at (m.top) {};
      \node[twfrobcup, anchor=leftleg] (cup) at (m.rightleg) {};
      \node[identity, anchor=top] at (m'.rightleg) {};
      \idstack[anchor=m.leftleg]{2}
      \node[twfrobcup, anchor=rightleg] (cup') at (id2.bottom) {};
      \node[twfrobcap, anchor=leftleg] (cap) at (m'.top) {};
      \idstack[anchor=cap.rightleg]{6}
      \idstack[anchor=cup'.leftleg, direction=up]{6}
      \node[draw=red, dashed, fit={(m'.top) (m.leftleg) (cup.bottom) (m'.rightleg)}]{};
    \end{tikzpicture}
    };
  \node (4) at (336.5bp,384.5bp) [] {
    \begin{tikzpicture}[baseline=(current bounding box.center)]
      \node[twfrobcup, anchor=rightleg] (cup'){};
      \node[twfrobcap, anchor=leftleg] (cap) at (cup'.rightleg) {};
      \idstack[anchor=cap.rightleg]{1}
      \node[comult, dot=black, anchor=rightleg, span=3.5] (c) at (id1.bottom) {};
      \idstack[anchor=cup'.leftleg, direction=up]{1}
      \node[comult, anchor=bottom] (c') at (id1.top) {};
      \node[twfrobcap, anchor=rightleg] (cap') at (c'.leftleg) {};
      \draw (cap'.leftleg) -- (c.leftleg);
      \idstack[anchor=c'.rightleg, direction=up]{2}
    \end{tikzpicture}
    };
  \node (7) at (336.5bp,218.5bp) [] {
    \begin{tikzpicture}[baseline=(current bounding box.center)]
      \node[mult] (m) {};
      \node[mult, dot=black, anchor=leftleg, span=1.5] (m') at (m.top) {};
      \node[twfrobcup, anchor=leftleg] (cup) at (m.rightleg) {};
      \node[identity, anchor=top] at (m'.rightleg) {};
      \idstack[anchor=m.leftleg]{1}
      \node[twfrobcup, anchor=rightleg] (cup') at (id1.bottom) {};
      \node[twfrobcap, anchor=leftleg] (cap') at (m'.top) {};
      \node[twfrobcap, anchor=rightleg] (cap'') at (cup'.leftleg) {};
      \idstack[anchor=cap''.leftleg]{1}
      \node[mult, anchor=top] (m''') at (id1.bottom) {};
      \node[twfrobcup, anchor=rightleg] (cup''') at (m'''.leftleg) {};
      \node[twfrobcup, anchor=leftleg] (cup'') at (cap'.rightleg) {};
      \node[mult, dot=black, anchor=leftleg] (m'') at (cup''.rightleg) {};
      \node[twfrobcap, anchor=leftleg] (cap) at (m''.top) {};
      \idstack[anchor=cap.rightleg]{8}
      \idstack[anchor=m''.rightleg]{2}
      \node[swishl, anchor=top] (s) at (id2.bottom) {};
      \node[swishl, anchor=top] (s) at (s.bottom) {};
      \node[swishl, anchor=top] (s) at (s.bottom) {};
      \node[twfrobcup, anchor=leftleg, span=2.75] (cup'''') at (m'''.rightleg) {};
      \draw (cup''''.rightleg) -- (s.bottom);
      \idstack[anchor=cup'''.leftleg, direction=up]{8}
    \end{tikzpicture}
    };
  \node (6) at (995.5bp,361.5bp) [] {
    \begin{tikzpicture}[baseline=(current bounding box.center)]
      \node[twfrobcup, anchor=rightleg] (cup) {};
      \node[twfrobcap, anchor=leftleg] (cap) at (cup.rightleg) {};
      \idstack[anchor=cap.rightleg]{2}
      \idstack[anchor=cup.leftleg, direction=up]{2}
    \end{tikzpicture}
    };
  \node (8) at (502.5bp,218.5bp) [] {
    \begin{tikzpicture}[baseline=(current bounding box.center)]
      \node[mult] (m) {};
      \node[mult, dot=black, anchor=leftleg, span=1.5] (m') at (m.top) {};
      \node[twfrobcup, anchor=leftleg] (cup) at (m.rightleg) {};
      \node[identity, anchor=top] at (m'.rightleg) {};
      \idstack[anchor=m.leftleg]{1}
      \node[mult, anchor=top] (m''') at (id1.bottom) {};
      \node[twfrobcup, anchor=rightleg] (cup''') at (m'''.leftleg) {};
      \node[mult, dot=black, anchor=leftleg] (m'') at (m'.top) {};
      \node[twfrobcap, anchor=leftleg] (cap) at (m''.top) {};
      \idstack[anchor=cap.rightleg]{7}
      \idstack[anchor=m''.rightleg]{4}
      \node[twfrobcup, anchor=leftleg, span=1.75] (cup'''') at (m'''.rightleg) {};
      \draw (cup''''.rightleg) -- (id4.bottom);
      \idstack[anchor=cup'''.leftleg, direction=up]{7}
      \node[draw=red, dashed, fit={(m'.top) (m.leftleg) (cup.bottom) (m'.rightleg)}]{};
      \node[draw=blue, dashed, fit={(m'''.leftleg) (m.top) (m.rightleg)}]{};
      \node[draw=blue, dashed, fit={(m'.leftleg) (m''.top) (m''.rightleg)}]{};
    \end{tikzpicture}
    };
  \node (9) at (663.0bp,178.5bp) [] {
    \begin{tikzpicture}[baseline=(current bounding box.center)]
      \node[mult] (m) {};
      \node[mult, dot=black, anchor=leftleg, span=2.5] (m') at (m.top) {};
      \node[mult, anchor=top] (m''') at (m.rightleg) {};
      \node[twfrobcup, anchor=rightleg] (cup''') at (m.leftleg) {};
      \node[mult, dot=black, anchor=top] (m'') at (m'.rightleg) {};
      \node[twfrobcap, anchor=leftleg, span=2] (cap) at (m'.top) {};
      \idstack[anchor=cap.rightleg]{8}
      \node[twfrobcup, anchor=leftleg] (cup'''') at (m'''.rightleg) {};
      \idstack[anchor=m'''.leftleg]{1}
      \node[swishr, anchor=top] (s) at (id1.bottom) {};
      \node[twfrobcup, anchor=leftleg, span=2] (cup'') at (s.bottom) {};
      \draw (cup''''.rightleg) -- (m''.leftleg);
      \draw (cup''.rightleg) -- (m''.rightleg);
      \idstack[anchor=cup'''.leftleg, direction=up]{5}
    \end{tikzpicture}
    };
  \node (10) at (775.0bp,178.5bp) [] {
    \begin{tikzpicture}[baseline=(current bounding box.center)]
      \node[mult] (m) {};
      \node[mult, dot=black, anchor=leftleg, span=1.5] (m') at (m.top) {};
      \node[mult, anchor=top] (m''') at (m.rightleg) {};
      \idstack[anchor=m.leftleg]{3}
      \node[twfrobcup, anchor=rightleg] (cup''') at (id3.bottom) {};
      \node[comult, dot=black, anchor=leftleg] (c) at (m'''.leftleg) {};
      \node[twfrobcap, anchor=leftleg] (cap) at (m'.top) {};
      \idstack[anchor=cap.rightleg]{7}
      \node[twfrobcup, anchor=leftleg] (cup'') at (c.bottom) {};
      \draw (cup''.rightleg) -- (m'.rightleg);
      \idstack[anchor=cup'''.leftleg, direction=up]{7}
      \node[draw=red, dashed, fit={(m'''.top) (c.bottom) (m'''.rightleg) (c.leftleg)}]{};
    \end{tikzpicture}
    };
  \node (11) at (896.0bp,178.5bp) [] {
    \begin{tikzpicture}[baseline=(current bounding box.center)]
      \node[mult] (m) {};
      \node[mult, dot=black, anchor=leftleg, span=1.5] (m') at (m.top) {};
      \node[twfrobcup, anchor=leftleg] (cup) at (m.rightleg) {};
      \node[identity, anchor=top] at (m'.rightleg) {};
      \idstack[anchor=m.leftleg]{2}
      \node[twfrobcup, anchor=rightleg] (cup') at (id2.bottom) {};
      \node[twfrobcap, anchor=leftleg] (cap) at (m'.top) {};
      \idstack[anchor=cap.rightleg]{6}
      \idstack[anchor=cup'.leftleg, direction=up]{6}
      \node[draw=red, dashed, fit={(m'.top) (m.leftleg) (cup.bottom) (m'.rightleg)}]{};
    \end{tikzpicture}
    };
  \node (13) at (336.5bp,55.5bp) [] {
    \begin{tikzpicture}[baseline=(current bounding box.center)]
      \node[comult, dot=black, span=1.5] (c) {};
      \node[comult, anchor=bottom] (c'') at (c.rightleg) {};
      \node[comult, anchor=bottom] (c''') at (c''.leftleg) {};
      \node[mult, dot=black, anchor=leftleg] (m) at (c'''.leftleg) {};
      \node[twfrobcap, anchor=rightleg] (cap) at (m.top) {};
      \draw (cap.leftleg) -- (c.leftleg);
      \idstack[anchor=c''.rightleg, direction=up]{4}
      \node[draw=red, dashed, fit={(m.top) (c'''.bottom) (m.rightleg) (c'''.leftleg)}]{};
    \end{tikzpicture}
    };
  \node (14) at (580.5bp,55.5bp) [] {
    \begin{tikzpicture}[baseline=(current bounding box.center)]
      \node[comult] (c) {};
      \node[twfrobcap, anchor=rightleg] (cap) at (c.leftleg) {};
      \node[comult, dot=black, anchor=rightleg, span=1.5] (c') at (c.bottom) {};
      \idstack[anchor=cap.leftleg]{1}
      \idstack[anchor=c.rightleg, direction=up]{2}
    \end{tikzpicture}
    };
  \draw [->,>=Implies,double equal sign distance] (0) ..controls (74.134bp,396.76bp) and (98.95bp,421.87bp)  .. (127.0bp,435.5bp) .. controls (240.34bp,490.56bp) and (285.57bp,472.38bp)  .. (410.0bp,452.5bp) .. controls (431.53bp,449.06bp) and (454.87bp,441.34bp)  .. node[auto] {\textcolor{red}{$\LTr$}} (1);
  \definecolor{strokecol}{rgb}{0.0,0.0,0.0};
  \pgfsetstrokecolor{strokecol}
  \draw (62.763bp,369.78bp) node[auto] {$$};
  \draw (476.31bp,424.77bp) node[auto] {$$};
  \draw [->,>=Implies,double equal sign distance] (0) ..controls (76.537bp,340.5bp) and (97.522bp,340.5bp)  .. node[auto] {$$} (3);
  \draw [->,>=Implies,double equal sign distance] (0) ..controls (79.401bp,275.73bp) and (112.33bp,231.67bp)  .. node[right] {$\textcolor{blue}{\alpha}$} node[left] {$\textcolor{blue}{\alpha}$} (12);
  \draw (62.819bp,299.95bp) node[right] {$$};
  \draw (136.9bp,184.77bp) node[right] {$$};
  \draw [->,>=Implies,double equal sign distance] (1) ..controls (552.12bp,441.29bp) and (610.5bp,460.5bp)  .. (662.0bp,460.5bp) .. controls (662.0bp,460.5bp) and (662.0bp,460.5bp)  .. (996.5bp,460.5bp) .. controls (1019.2bp,460.5bp) and (1037.6bp,438.71bp)  .. node[auto] {$\LTr$} (2);
  \draw (528.67bp,424.19bp) node[auto] {$$};
  \draw (1047.0bp,409.11bp) node[auto] {$$};
  \draw [->,>=Implies,double equal sign distance] (1) ..controls (547.66bp,405.51bp) and (590.94bp,388.85bp)  .. node[auto] {$$} (5);
  \draw [->,>=Implies,double equal sign distance] (3) ..controls (239.13bp,358.57bp) and (269.2bp,366.66bp)  .. node[auto] {\textcolor{red}{$\RTr$}} (4);
  \draw (220.96bp,346.06bp) node[auto] {$$};
  \draw (297.16bp,369.8bp) node[auto] {$$};
  \draw [->,>=Implies,double equal sign distance] (3) ..controls (228.41bp,298.41bp) and (247.26bp,284.34bp)  .. node[auto] {$$} (7);
  \draw [->,>=Implies,double equal sign distance] (4) ..controls (399.66bp,398.9bp) and (443.39bp,409.04bp)  .. node[auto] {$$} (1);
  \draw [->,>=Implies,double equal sign distance] (5) ..controls (757.19bp,361.5bp) and (901.9bp,361.5bp)  .. node[auto] {\textcolor{red}{$\RTr$}} (6);
  \draw (700.21bp,355.5bp) node[auto] {$$};
  \draw (968.98bp,355.5bp) node[auto] {$$};
  \draw [->,>=Implies,double equal sign distance] (6) ..controls (1024.5bp,384.72bp) and (1036.5bp,394.68bp)  .. node[auto] {$$} (2);
  \draw [->,>=Implies,double equal sign distance] (7) ..controls (424.7bp,218.5bp) and (439.38bp,218.5bp)  .. node[auto] {$$} (8);
  \draw [->,>=Implies,double equal sign distance] (8) ..controls (564.82bp,273.83bp) and (600.36bp,305.89bp)  .. node[auto] {\textcolor{red}{$\RTr$}} (5);
  \draw (544.68bp,244.24bp) node[auto] {$$};
  \draw (628.04bp,330.27bp) node[auto] {$$};
  \draw [->,>=Implies,double equal sign distance] (8) ..controls (562.13bp,203.7bp) and (587.3bp,197.35bp)  .. node[below] {$\textcolor{blue}{\alpha}$} node[above] {$\textcolor{blue}{\alpha}$} (9);
  \draw (547.87bp,202.82bp) node[below] {$$};
  \draw (613.24bp,183.29bp) node[below] {$$};
  \draw [->,>=Implies,double equal sign distance] (9) ..controls (715.89bp,178.5bp) and (725.04bp,178.5bp)  .. node[auto] {$$} (10);
  \draw [->,>=Implies,double equal sign distance] (10) ..controls (820.83bp,178.5bp) and (838.88bp,178.5bp)  .. node[auto] {\textcolor{red}{$\varepsilon_\otimes$}} (11);
  \draw (812.03bp,172.5bp) node[auto] {$$};
  \draw (858.98bp,172.5bp) node[auto] {$$};
  \draw [->,>=Implies,double equal sign distance] (11) ..controls (937.33bp,254.2bp) and (960.01bp,296.77bp)  .. node[auto] {$\textcolor{red}{\RTr}$} (6);
  \draw (926.35bp,216.33bp) node[auto] {$$};
  \draw (974.67bp,329.54bp) node[auto] {$$};
  \draw [->,>=Implies,double equal sign distance] (12) ..controls (233.24bp,117.42bp) and (278.42bp,90.061bp)  .. node[auto] {$$} (13);
  \draw [->,>=Implies,double equal sign distance] (13) ..controls (399.69bp,55.5bp) and (499.39bp,55.5bp)  .. node[auto] {$\textcolor{red}{\varepsilon_\invamp}$} (14);
  \draw (363.3bp,49.5bp) node[auto] {$$};
  \draw (553.76bp,49.5bp) node[auto] {$$};
  \draw [->,>=Implies,double equal sign distance] (14) ..controls (641.61bp,53.561bp) and (736.89bp,55.396bp)  .. (806.0bp,90.5bp) .. controls (827.34bp,101.34bp) and (846.79bp,119.14bp)  .. node[auto] {$$} (11);
%
\end{tikzpicture}


==> main-dot2tex-fig2.tex <==
%%
\node (0) at (19.5bp,77.0bp) [] {
        \begin{tikzpicture}[baseline=(current bounding box.center)]
          \node[comult] (c) {};
          \node[comult, dot=black, anchor=bottom] (m) at (c.rightleg) {};
          \node[identity, anchor=bottom] (i) at (c.leftleg) {};
          \node[draw=red, dashed, fit={(m.leftleg) (i.top)}]{};
          \node[draw=blue, dashed, fit={(m.leftleg) (m.rightleg)}]{};
        \end{tikzpicture}
        };
  \node (1) at (122.0bp,173.0bp) [] {
        \begin{tikzpicture}[baseline=(current bounding box.center)]
          \node[comult, span=1.5] (c) {};
          \node[comult, dot=black, anchor=bottom] (m) at (c.rightleg) {};
          \node[identity, anchor=bottom] at (c.leftleg) {};
          \node[mult, dot=black, anchor=rightleg] (m') at (m.leftleg) {};
          \node[comult, anchor=bottom] (c') at (m'.top) {};
          \idstack[anchor=m.rightleg, direction=up]{2}
          \node[draw=red, dashed, fit={(m'.north) (m.rightleg) (m'.leftleg) (m.south)}]{};
          \node[draw=blue, dashed, fit={(id2.top) (c'.rightleg)}]{};
        \end{tikzpicture}
        };
  \node (30) at (122.0bp,77.0bp) [] {
        \begin{tikzpicture}[baseline=(current bounding box.center)]
          \node[comult] (c) {};
          \node[comult, dot=black, anchor=bottom] (c') at (c.rightleg) {};
          \idstack[anchor=c.leftleg, direction=up]{3}
          \node[mult, anchor=leftleg] (tm) at (c'.leftleg) {};
          \node[comult, dot=black, anchor=bottom] (tc) at (tm.top) {};
          \node[draw=red, dashed, fit={(id1.top) (tm.leftleg)}]{};
          \node[draw=blue, dashed, fit={(tm.north) (tm.leftleg) (c'.south) (c'.rightleg)}]{};
        \end{tikzpicture}
        };
  \node (40) at (359.0bp,30.0bp) [] {
        \begin{tikzpicture}[baseline=(current bounding box.center)]
          \node[comult] (c) {};
          \idstack[anchor=c.leftleg, direction=up]{1}
          \node[comult, dot=black, anchor=bottom] (c') at (c.rightleg) {};
          \node[draw=red, dashed, fit={(c.leftleg) (c.rightleg)}]{};
        \end{tikzpicture}
        };
  \node (2) at (280.0bp,246.0bp) [] {
        \begin{tikzpicture}[baseline=(current bounding box.center)]
          \node[comult, dot=black] (c) {};
          \node[comult, anchor=bottom] (m) at (c.leftleg) {};
          \node[mult, dot=black, anchor=top] (m') at (c.bottom) {};
          \node[comult, anchor=rightleg] (c') at (m'.rightleg) {};
          \idstack[anchor=c.rightleg, direction=up]{1}
          \node[draw=red, dashed, fit={(m'.north) (m'.rightleg) (m'.leftleg) (c'.south)}]{};
          \node[draw=blue, dashed, fit={(m.rightleg) (id1.top)}]{};
        \end{tikzpicture}
        };
  \node (20) at (280.0bp,133.0bp) [] {
        \begin{tikzpicture}[baseline=(current bounding box.center)]
          \node[comult, span=1.5] (c) {};
          \node[comult, dot=black, anchor=bottom] (m) at (c.rightleg) {};
          \node[identity, anchor=bottom] at (c.leftleg) {};
          \node[mult, dot=black, anchor=rightleg] (m') at (m.leftleg) {};
          \node[comult, anchor=bottom] (c') at (m'.top) {};
          \idstack[anchor=m.rightleg, direction=up]{2}
          \node[draw=red, dashed, fit={(m'.north) (m.rightleg) (m'.leftleg) (m.south)}]{};
          \idstack[anchor=c'.leftleg, direction=up]{2}
          \node[mult, anchor=leftleg] (tm) at (c'.rightleg) {};
          \node[comult, dot=black, anchor=bottom] (tc) at (tm.top) {};
          \node[draw=blue, dashed, fit={(tm.north) (c'.south) (tm.rightleg) (c'.leftleg)}]{};
        \end{tikzpicture}
        };
  \node (3) at (469.5bp,292.0bp) [] {
        \begin{tikzpicture}[baseline=(current bounding box.center)]
          \node[comult, dot=black] (c) {};
          \node[comult, anchor=bottom] (m) at (c.leftleg) {};
          \idstack[anchor=c.rightleg, direction=up]{1}
          \node[draw=red, dashed, fit={(m.rightleg) (id1.top)}]{};
        \end{tikzpicture}
        };
  \node (10) at (469.5bp,196.0bp) [] {
        \begin{tikzpicture}[baseline=(current bounding box.center)]
          \node[comult, dot=black, span=1.5] (c) {};
          \node[comult, anchor=bottom] (m) at (c.leftleg) {};
          \node[identity, anchor=bottom] at (c.rightleg) {};
          \node[mult, anchor=leftleg] (m') at (m.rightleg) {};
          \node[comult, dot=black, anchor=bottom] (c') at (m'.top) {};
          \node[mult, dot=black, anchor=top] (bm) at (c.bottom) {};
          \node[comult, anchor=leftleg] (bc) at (bm.leftleg) {};
          \idstack[anchor=m.leftleg, direction=up]{2}
          \node[draw=blue, dashed, fit={(m.leftleg) (m.south) (m'.rightleg) (m'.north)}]{};
          \node[draw=red, dashed, fit={(bm.north) (bm.leftleg) (bc.rightleg) (bc.south)}]{};
        \end{tikzpicture}
        };
  \node (4) at (696.0bp,232.0bp) [] {
        \begin{tikzpicture}[baseline=(current bounding box.center)]
          \node[comult, dot=black, span=1.5] (c) {};
          \node[comult, anchor=bottom] (m) at (c.leftleg) {};
          \node[identity, anchor=bottom] at (c.rightleg) {};
          \node[mult, anchor=leftleg] (m') at (m.rightleg) {};
          \node[comult, dot=black, anchor=bottom] (c') at (m'.top) {};
          \idstack[anchor=m.leftleg, direction=up]{2}
          \node[draw=red, dashed, fit={(m.leftleg) (m.south) (m'.rightleg) (m'.north)}]{};
        \end{tikzpicture}
        };
  \node (5) at (885.0bp,159.0bp) [] {
        \begin{tikzpicture}[baseline=(current bounding box.center)]
          \node[comult] (c) {};
          \node[comult, dot=black, anchor=bottom] (c') at (c.rightleg) {};
          \node[mult, anchor=top] (m) at (c.bottom) {};
          \node[comult, dot=black, anchor=leftleg] (c'') at (m.leftleg) {};
          \node[draw=red, dashed, fit={(m.north) (c''.south) (m.rightleg) (c''.leftleg)}]{};
          \idstack[anchor=c.leftleg, direction=up]{1}
        \end{tikzpicture}
        };
  \node (6) at (978.5bp,66.0bp) [] {
        \begin{tikzpicture}[baseline=(current bounding box.center)]
          \node[comult] (c) {};
          \node[comult, dot=black, anchor=bottom] (m) at (c.rightleg) {};
          \node[identity, anchor=bottom] (i) at (c.leftleg) {};
        \end{tikzpicture}
        };
  \node (11) at (696.0bp,121.0bp) [] {
        \begin{tikzpicture}[baseline=(current bounding box.center)]
          \node[comult] (c) {};
          \node[comult, dot=black, anchor=bottom] (c') at (c.rightleg) {};
          \node[mult, anchor=top] (m) at (c.bottom) {};
          \node[comult, dot=black, anchor=leftleg] (c'') at (m.leftleg) {};
          \node[draw=blue, dashed, fit={(m.north) (c''.south) (m.rightleg) (c''.leftleg)}]{};
          \idstack[anchor=c.leftleg, direction=up]{1}
          \node[mult, dot=black, anchor=top] (bm) at (c''.bottom) {};
          \node[comult, anchor=leftleg] (bc) at (bm.leftleg) {};
          \node[draw=red, dashed, fit={(bm.north) (bc.south) (bm.rightleg) (bc.leftleg)}]{};
        \end{tikzpicture}
        };
  \node (41) at (885.0bp,66.0bp) [] {
        \begin{tikzpicture}[baseline=(current bounding box.center)]
          \node[comult] (c) {};
          \node[mult, dot=black, anchor=leftleg] (m) at (c.leftleg) {};
          \node[comult, anchor=bottom] (c') at (m.top) {};
          \idstack[anchor=c'.leftleg, direction=up]{1}
          \node[comult, dot=black, anchor=bottom] (c'') at (c'.rightleg) {};
          \node[draw=red, dashed, fit={(c.south) (c.leftleg) (m.rightleg) (m.north)}]{};
        \end{tikzpicture}
        };
  \draw [->,>=Implies,double equal sign distance] (0) ..controls (50.069bp,105.24bp) and (74.334bp,128.42bp)  .. node[auto] {$\textcolor{red}{\eta_\invamp}$} (1);
  \definecolor{strokecol}{rgb}{0.0,0.0,0.0};
  \pgfsetstrokecolor{strokecol}
  \draw (40.899bp,96.754bp) node[auto] {$$};
  \draw (94.717bp,147.63bp) node[auto] {$$};
  \draw [->,>=Implies,double equal sign distance] (0) ..controls (54.142bp,77.0bp) and (74.873bp,77.0bp)  .. node[auto] {$\textcolor{blue}{\eta_\otimes}$} (30);
  \draw (45.403bp,71.0bp) node[auto] {$$};
  \draw (96.181bp,71.0bp) node[auto] {$$};
  \draw [->,tips=false,double equal sign distance] (0) ..controls (50.539bp,53.364bp) and (74.323bp,37.546bp)  .. (98.0bp,31.0bp) .. controls (180.34bp,8.2335bp) and (283.04bp,18.582bp)  .. node[auto] {$$} (40);
  \draw [->,tips=false,double equal sign distance] (1) ..controls (173.78bp,196.76bp) and (222.8bp,219.7bp)  .. node[auto] {$\textcolor{red}{\labelcref{eq:frobenius}}$} (2);
  \draw (151.35bp,177.46bp) node[auto] {$$};
  \draw (255.97bp,232.03bp) node[auto] {$$};
  \draw [->,>=Implies,double equal sign distance] (1) ..controls (172.4bp,160.33bp) and (215.86bp,149.19bp)  .. node[auto] {$\textcolor{blue}{\eta_\otimes}$} (20);
  \draw (152.02bp,161.1bp) node[auto] {$$};
  \draw (249.89bp,132.93bp) node[auto] {$$};
  \draw [->,>=Implies,double equal sign distance] (2) ..controls (330.67bp,258.19bp) and (402.63bp,275.84bp)  .. node[auto] {$\textcolor{red}{\varepsilon_\invamp}$} (3);
  \draw (303.97bp,256.16bp) node[auto] {$$};
  \draw (445.7bp,281.88bp) node[auto] {$$};
  \draw [->,>=Implies,double equal sign distance] (2) ..controls (305.5bp,239.42bp) and (314.17bp,237.09bp)  .. (322.0bp,235.0bp) .. controls (361.01bp,224.57bp) and (405.88bp,212.64bp)  .. node[auto] {$\textcolor{blue}{\eta_\otimes}$} (10);
  \draw (304.15bp,235.39bp) node[auto] {$$};
  \draw (439.41bp,196.13bp) node[auto] {$$};
  \draw [->,>=Implies,double equal sign distance] (3) ..controls (519.78bp,280.99bp) and (593.21bp,263.96bp)  .. (654.0bp,246.0bp) .. controls (656.77bp,245.18bp) and (659.64bp,244.29bp)  .. node[auto] {$\textcolor{red}{\eta_\otimes}$} (4);
  \draw (493.33bp,282.28bp) node[auto] {$$};
  \draw (666.12bp,234.19bp) node[auto] {$$};
  \draw [->,>=Implies,double equal sign distance] (4) ..controls (754.27bp,209.64bp) and (820.65bp,183.73bp)  .. node[auto] {$\textcolor{red}{\labelcref{eq:white-frobenius}}$} (5);
  \draw (725.56bp,217.19bp) node[auto] {$$};
  \draw (861.15bp,159.58bp) node[auto] {$$};
  \draw [->,>=Implies,double equal sign distance] (5) ..controls (917.09bp,127.4bp) and (941.1bp,103.0bp)  .. node[auto] {$\textcolor{red}{\varepsilon_\otimes}$} (6);
  \draw (907.52bp,137.22bp) node[auto] {$$};
  \draw (959.14bp,84.567bp) node[auto] {$$};
  \draw [->,>=Implies,double equal sign distance] (10) ..controls (533.69bp,206.13bp) and (615.85bp,219.31bp)  .. node[auto] {$\textcolor{red}{\varepsilon_\invamp}$} (4);
  \draw (499.68bp,193.72bp) node[auto] {$$};
  \draw (665.95bp,222.3bp) node[auto] {$$};
  \draw [->,>=Implies,double equal sign distance] (10) ..controls (535.67bp,174.23bp) and (624.07bp,144.7bp)  .. node[auto] {$\textcolor{blue}{\labelcref{eq:white-frobenius}}$} (11);
  \draw (499.68bp,182.26bp) node[auto] {$$};
  \draw (671.95bp,132.7bp) node[auto] {$$};
  \draw [->,>=Implies,double equal sign distance] (11) ..controls (746.9bp,131.14bp) and (817.92bp,145.57bp)  .. node[auto] {$\textcolor{red}{\varepsilon_\invamp}$} (5);
  \draw (720.26bp,118.51bp) node[auto] {$$};
  \draw (861.05bp,149.56bp) node[auto] {$$};
  \draw [->,>=Implies,double equal sign distance] (11) ..controls (721.46bp,113.11bp) and (730.14bp,110.38bp)  .. (738.0bp,108.0bp) .. controls (779.37bp,95.492bp) and (827.6bp,81.787bp)  .. node[auto] {$\textcolor{blue}{\varepsilon_\otimes}$} (41);
  \draw (720.12bp,109.46bp) node[auto] {$$};
  \draw (860.87bp,64.765bp) node[auto] {$$};
  \draw [->,tips=false,double equal sign distance] (20) ..controls (337.12bp,151.85bp) and (398.41bp,172.45bp)  .. node[auto] {$\textcolor{red}{\labelcref{eq:frobenius}}$} (10);
  \draw (309.99bp,134.73bp) node[auto] {$$};
  \draw (439.61bp,182.31bp) node[auto] {$$};
  \draw [->,>=Implies,double equal sign distance] (20) ..controls (330.36bp,115.34bp) and (374.58bp,101.38bp)  .. (414.0bp,96.0bp) .. controls (506.68bp,83.349bp) and (617.47bp,103.49bp)  .. node[above] {$\textcolor{blue}{\labelcref{eq:white-frobenius}}$} node[below] {$\textcolor{red}{\labelcref{eq:frobenius}}$} (11);
  \draw (310.14bp,118.49bp) node[above] {$$};
  \draw (671.83bp,110.8bp) node[above] {$$};
  \draw [->,>=Implies,double equal sign distance] (30) ..controls (167.36bp,92.925bp) and (214.68bp,109.91bp)  .. node[auto] {$\textcolor{red}{\eta_\invamp}$} (20);
  \draw (147.51bp,77.644bp) node[auto] {$$};
  \draw (250.23bp,118.82bp) node[auto] {$$};
  \draw [->,>=Implies,double equal sign distance] (30) ..controls (182.78bp,65.043bp) and (283.03bp,44.994bp)  .. node[auto] {$\textcolor{blue}{\varepsilon_\otimes}$} (40);
  \draw (147.44bp,67.312bp) node[auto] {$$};
  \draw (335.23bp,39.353bp) node[auto] {$$};
  \draw [->,tips=false,double equal sign distance] (40) ..controls (415.69bp,18.402bp) and (514.17bp,0.0000bp)  .. (597.5bp,0.0bp) .. controls (597.5bp,0.0bp) and (597.5bp,0.0bp)  .. (886.0bp,0.0bp) .. controls (916.51bp,0.0bp) and (943.76bp,24.43bp)  .. node[auto] {$$} (6);
  \draw [->,>=Implies,double equal sign distance] (40) ..controls (453.49bp,36.423bp) and (763.02bp,57.689bp)  .. node[auto] {$\textcolor{red}{\eta_\invamp}$} (41);
  \draw (383.14bp,25.177bp) node[auto] {$$};
  \draw (860.99bp,58.832bp) node[auto] {$$};
  \draw [->,>=Implies,double equal sign distance] (41) ..controls (916.92bp,66.0bp) and (936.33bp,66.0bp)  .. node[auto] {$\textcolor{red}{\varepsilon_\invamp}$} (6);
  \draw (909.21bp,60.0bp) node[auto] {$$};
  \draw (955.89bp,60.0bp) node[auto] {$$};
%

==> main-dot2tex-fig3.tex <==
%%
\node (0) at (19.5bp,77.0bp) [] {
        \begin{tikzpicture}[baseline=(current bounding box.center)]
          \node[comult, dot=black] (c) {};
          \node[comult, anchor=bottom] (c') at (c.leftleg) {};
          \idstack[anchor=c.rightleg, direction=up]{1}
          \node[draw=red, dashed, fit={(c'.rightleg) (id1.top)}]{};
          \node[draw=blue, dashed, fit={(c'.leftleg) (c'.rightleg)}]{};
        \end{tikzpicture}
        };
  \node (1) at (122.0bp,173.0bp) [] {
        \begin{tikzpicture}[baseline=(current bounding box.center)]
          \node[comult, dot=black, span=1.5] (c) {};
          \node[comult, anchor=bottom] (m) at (c.leftleg) {};
          \node[identity, anchor=bottom] at (c.rightleg) {};
          \node[mult, anchor=leftleg] (m') at (m.rightleg) {};
          \node[comult, dot=black, anchor=bottom] (c') at (m'.top) {};
          \idstack[anchor=m.leftleg, direction=up]{2}
          \node[draw=red, dashed, fit={(m.leftleg) (m.south) (m'.rightleg) (m'.north)}]{};
          \node[draw=blue, dashed, fit={(id2.top) (c'.leftleg)}]{};
        \end{tikzpicture}
        };
  \node (30) at (122.0bp,77.0bp) [] {
        \begin{tikzpicture}[baseline=(current bounding box.center)]
          \node[comult, dot=black] (c) {};
          \node[comult, anchor=bottom] (c') at (c.leftleg) {};
          \idstack[anchor=c.rightleg, direction=up]{3}
          \node[mult, dot=black, anchor=leftleg] (tm) at (c'.leftleg) {};
          \node[comult, anchor=bottom] (tc) at (tm.top) {};
          \node[draw=red, dashed, fit={(c'.rightleg) (id1.top)}]{};
          \node[draw=blue, dashed, fit={(tm.north) (tm.leftleg) (c'.rightleg) (c'.south)}]{};
        \end{tikzpicture}
        };
  \node (40) at (414.5bp,30.0bp) [] {
        \begin{tikzpicture}[baseline=(current bounding box.center)]
          \node[comult, dot=black] (c) {};
          \node[comult, anchor=bottom] (c') at (c.leftleg) {};
          \idstack[anchor=c.rightleg, direction=up]{1}
          \node[draw=red, dashed, fit={(c.leftleg) (c.rightleg)}]{};
        \end{tikzpicture}
        };
  \node (2) at (317.0bp,246.0bp) [] {
        \begin{tikzpicture}[baseline=(current bounding box.center)]
          \node[comult] (c) {};
          \node[comult, dot=black, anchor=bottom] (c') at (c.rightleg) {};
          \node[mult, anchor=top] (m) at (c.bottom) {};
          \node[comult, dot=black, anchor=leftleg] (c'') at (m.leftleg) {};
          \node[draw=red, dashed, fit={(m.north) (c''.south) (m.rightleg) (c''.leftleg)}]{};
          \idstack[anchor=c.leftleg, direction=up]{1}
          \node[draw=blue, dashed, fit={(id1.top) (c'.leftleg)}]{};
        \end{tikzpicture}
        };
  \node (20) at (317.0bp,133.0bp) [] {
        \begin{tikzpicture}[baseline=(current bounding box.center)]
          \node[comult, dot=black, span=1.5] (c) {};
          \node[comult, anchor=bottom] (m) at (c.leftleg) {};
          \node[identity, anchor=bottom] at (c.rightleg) {};
          \node[mult, anchor=leftleg] (m') at (m.rightleg) {};
          \node[comult, dot=black, anchor=bottom] (c') at (m'.top) {};
          \idstack[anchor=m.leftleg, direction=up]{2}
          \node[draw=red, dashed, fit={(m.leftleg) (m.south) (m'.rightleg) (m'.north)}]{};
          \idstack[anchor=c'.rightleg, direction=up]{1}
          \node[mult, dot=black, anchor=rightleg] (tm) at (c'.leftleg) {};
          \node[comult, anchor=bottom] (tc) at (tm.top) {};
          \node[draw=blue, dashed, fit={(c'.rightleg) (c'.south) (tm.leftleg) (tm.north)}]{};
        \end{tikzpicture}
        };
  \node (3) at (543.5bp,292.0bp) [] {
        \begin{tikzpicture}[baseline=(current bounding box.center)]
          \node[comult] (c) {};
          \node[comult, dot=black, anchor=bottom] (m) at (c.rightleg) {};
          \node[identity, anchor=bottom] (i) at (c.leftleg) {};
          \node[draw=red, dashed, fit={(m.leftleg) (i.top)}]{};
        \end{tikzpicture}
        };
  \node (10) at (543.5bp,196.0bp) [] {
        \begin{tikzpicture}[baseline=(current bounding box.center)]
          \node[comult, span=1.5] (c) {};
          \node[comult, dot=black, anchor=bottom] (m) at (c.rightleg) {};
          \node[identity, anchor=bottom] at (c.leftleg) {};
          \node[mult, dot=black, anchor=rightleg] (m') at (m.leftleg) {};
          \node[comult, anchor=bottom] (c') at (m'.top) {};
          \idstack[anchor=m.rightleg, direction=up]{2}
          \node[draw=blue, dashed, fit={(m'.north) (m.rightleg) (m'.leftleg) (m.south)}]{};
          \node[mult, anchor=top] (bm) at (c.bottom) {};
          \node[comult, dot=black, anchor=leftleg] (bc) at (bm.leftleg) {};
          \node[draw=red, dashed, fit={(bm.north) (bm.rightleg) (bc.leftleg) (bc.south)}]{};
        \end{tikzpicture}
        };
  \node (4) at (733.0bp,232.0bp) [] {
        \begin{tikzpicture}[baseline=(current bounding box.center)]
          \node[comult, span=1.5] (c) {};
          \node[comult, dot=black, anchor=bottom] (m) at (c.rightleg) {};
          \node[identity, anchor=bottom] at (c.leftleg) {};
          \node[mult, dot=black, anchor=rightleg] (m') at (m.leftleg) {};
          \node[comult, anchor=bottom] (c') at (m'.top) {};
          \idstack[anchor=m.rightleg, direction=up]{2}
          \node[draw=red, dashed, fit={(m'.north) (m.rightleg) (m'.leftleg) (m.south)}]{};
        \end{tikzpicture}
        };
  \node (5) at (885.0bp,159.0bp) [] {
        \begin{tikzpicture}[baseline=(current bounding box.center)]
          \node[comult, dot=black] (c) {};
          \node[comult, anchor=bottom] (m) at (c.leftleg) {};
          \node[mult, dot=black, anchor=top] (m') at (c.bottom) {};
          \node[comult, anchor=rightleg] (c') at (m'.rightleg) {};
          \idstack[anchor=c.rightleg, direction=up]{1}
          \node[draw=red, dashed, fit={(m'.north) (m'.rightleg) (m'.leftleg) (c'.south)}]{};
        \end{tikzpicture}
        };
  \node (6) at (978.5bp,66.0bp) [] {
        \begin{tikzpicture}[baseline=(current bounding box.center)]
          \node[comult, dot=black] (c) {};
          \node[comult, anchor=bottom] (m) at (c.leftleg) {};
          \idstack[anchor=c.rightleg, direction=up]{1}
        \end{tikzpicture}
        };
  \node (21) at (733.0bp,121.0bp) [] {
        \begin{tikzpicture}[baseline=(current bounding box.center)]
          \node[comult, dot=black] (c) {};
          \node[comult, anchor=bottom] (m) at (c.leftleg) {};
          \node[mult, dot=black, anchor=top] (m') at (c.bottom) {};
          \node[comult, anchor=rightleg] (c') at (m'.rightleg) {};
          \idstack[anchor=c.rightleg, direction=up]{1}
          \node[draw=blue, dashed, fit={(m'.north) (m'.rightleg) (m'.leftleg) (c'.south)}]{};
          \node[mult, anchor=top] (bm) at (c'.bottom) {};
          \node[comult, dot=black, anchor=leftleg] (bc) at (bm.leftleg) {};
          \node[draw=red, dashed, fit={(bm.north) (bm.leftleg) (bc.rightleg) (bc.south)}]{};
        \end{tikzpicture}
        };
  \node (31) at (885.0bp,66.0bp) [] {
        \begin{tikzpicture}[baseline=(current bounding box.center)]
          \node[comult, dot=black] (c) {};
          \node[comult, anchor=bottom] (m) at (c.leftleg) {};
          \node[mult, anchor=top] (m') at (c.bottom) {};
          \node[comult, dot=black, anchor=rightleg] (c') at (m'.rightleg) {};
          \idstack[anchor=c.rightleg, direction=up]{1}
          \node[draw=red, dashed, fit={(m'.north) (m'.rightleg) (m'.leftleg) (c'.south)}]{};
        \end{tikzpicture}
        };
  \draw [->,>=Implies,double equal sign distance] (0) ..controls (50.069bp,105.24bp) and (74.334bp,128.42bp)  .. node[auto] {$\textcolor{red}{\eta_\otimes}$} (1);
  \definecolor{strokecol}{rgb}{0.0,0.0,0.0};
  \pgfsetstrokecolor{strokecol}
  \draw (40.899bp,96.754bp) node[auto] {$$};
  \draw (94.717bp,147.63bp) node[auto] {$$};
  \draw [->,>=Implies,double equal sign distance] (0) ..controls (54.142bp,77.0bp) and (74.873bp,77.0bp)  .. node[auto] {$\textcolor{blue}{\eta_\otimes}$} (30);
  \draw (45.403bp,71.0bp) node[auto] {$$};
  \draw (96.181bp,71.0bp) node[auto] {$$};
  \draw [->,tips=false,double equal sign distance] (0) ..controls (50.537bp,53.358bp) and (74.321bp,37.538bp)  .. (98.0bp,31.0bp) .. controls (201.45bp,2.4338bp) and (331.37bp,17.01bp)  .. node[auto] {$$} (40);
  \draw [->,>=Implies,double equal sign distance] (1) ..controls (181.39bp,195.09bp) and (251.35bp,221.55bp)  .. node[auto] {$\textcolor{red}{\labelcref{eq:white-frobenius}}$} (2);
  \draw (151.52bp,175.52bp) node[auto] {$$};
  \draw (292.99bp,233.56bp) node[auto] {$$};
  \draw [->,>=Implies,double equal sign distance] (1) ..controls (179.9bp,161.21bp) and (243.93bp,147.94bp)  .. node[auto] {$\textcolor{blue}{\eta_\invamp}$} (20);
  \draw (151.9bp,162.25bp) node[auto] {$$};
  \draw (286.83bp,131.8bp) node[auto] {$$};
  \draw [->,>=Implies,double equal sign distance] (2) ..controls (374.11bp,257.5bp) and (468.78bp,276.9bp)  .. node[auto] {$\textcolor{red}{\varepsilon_\otimes}$} (3);
  \draw (341.24bp,243.53bp) node[auto] {$$};
  \draw (519.51bp,282.52bp) node[auto] {$$};
  \draw [->,>=Implies,double equal sign distance] (2) ..controls (342.31bp,237.02bp) and (351.01bp,234.14bp)  .. (359.0bp,232.0bp) .. controls (410.81bp,218.14bp) and (472.16bp,207.18bp)  .. node[auto] {$\textcolor{red}{\eta_\invamp}$} (10);
  \draw (341.0bp,233.62bp) node[auto] {$$};
  \draw (513.39bp,193.5bp) node[auto] {$$};
  \draw [->,>=Implies,double equal sign distance] (3) ..controls (592.21bp,276.73bp) and (659.52bp,255.19bp)  .. node[auto] {$\textcolor{red}{\eta_\invamp}$} (4);
  \draw (567.14bp,280.68bp) node[auto] {$$};
  \draw (703.37bp,233.24bp) node[auto] {$$};
  \draw [->,tips=false,double equal sign distance] (4) ..controls (783.37bp,207.97bp) and (829.53bp,185.51bp)  .. node[auto] {$\textcolor{red}{\labelcref{eq:frobenius}}$} (5);
  \draw (762.13bp,215.23bp) node[auto] {$$};
  \draw (861.35bp,161.1bp) node[auto] {$$};
  \draw [->,>=Implies,double equal sign distance] (5) ..controls (917.09bp,127.4bp) and (941.1bp,103.0bp)  .. node[auto] {$\textcolor{red}{\varepsilon_\invamp}$} (6);
  \draw (907.52bp,137.22bp) node[auto] {$$};
  \draw (959.14bp,84.567bp) node[auto] {$$};
  \draw [->,>=Implies,double equal sign distance] (10) ..controls (600.47bp,206.75bp) and (661.39bp,218.44bp)  .. node[auto] {$\textcolor{red}{\varepsilon_\otimes}$} (4);
  \draw (573.49bp,194.41bp) node[auto] {$$};
  \draw (703.11bp,221.61bp) node[auto] {$$};
  \draw [->,tips=false,double equal sign distance] (10) ..controls (602.35bp,172.86bp) and (668.42bp,146.43bp)  .. node[auto] {$\textcolor{blue}{\labelcref{eq:frobenius}}$} (21);
  \draw (573.49bp,180.8bp) node[auto] {$$};
  \draw (708.93bp,121.83bp) node[auto] {$$};
  \draw [->,>=Implies,double equal sign distance] (20) ..controls (381.28bp,150.76bp) and (463.7bp,173.89bp)  .. node[auto] {$\textcolor{red}{\labelcref{eq:white-frobenius}}$} (10);
  \draw (347.18bp,133.5bp) node[auto] {$$};
  \draw (513.45bp,183.53bp) node[auto] {$$};
  \draw [->,>=Implies,double equal sign distance] (20) ..controls (373.24bp,117.39bp) and (434.54bp,101.75bp)  .. (488.0bp,96.0bp) .. controls (537.05bp,90.724bp) and (549.88bp,91.423bp)  .. (599.0bp,96.0bp) .. controls (636.17bp,99.463bp) and (678.44bp,108.26bp)  .. node[above] {$\textcolor{blue}{\labelcref{eq:white-frobenius}}$} node[below] {$\textcolor{red}{\labelcref{eq:frobenius}}$} (21);
  \draw (346.84bp,120.39bp) node[above] {$$};
  \draw (708.93bp,110.74bp) node[above] {$$};
  \draw [->,>=Implies,double equal sign distance] (21) ..controls (777.09bp,131.92bp) and (826.27bp,144.38bp)  .. node[auto] {$\textcolor{red}{\varepsilon_\otimes}$} (5);
  \draw (757.21bp,119.36bp) node[auto] {$$};
  \draw (860.99bp,148.69bp) node[auto] {$$};
  \draw [->,>=Implies,double equal sign distance] (21) ..controls (776.8bp,105.31bp) and (826.46bp,87.098bp)  .. node[auto] {$\textcolor{blue}{\varepsilon_\invamp}$} (31);
  \draw (756.92bp,108.8bp) node[auto] {$$};
  \draw (860.92bp,78.264bp) node[auto] {$$};
  \draw [->,>=Implies,double equal sign distance] (30) ..controls (170.02bp,89.112bp) and (227.13bp,104.23bp)  .. (275.0bp,119.0bp) .. controls (277.76bp,119.85bp) and (280.62bp,120.76bp)  .. node[auto] {$\textcolor{red}{\eta_\invamp}$} (20);
  \draw (147.35bp,87.694bp) node[auto] {$$};
  \draw (287.09bp,118.91bp) node[auto] {$$};
  \draw [->,>=Implies,double equal sign distance] (30) ..controls (148.67bp,70.314bp) and (156.67bp,68.435bp)  .. (164.0bp,67.0bp) .. controls (244.37bp,51.275bp) and (340.46bp,38.78bp)  .. node[auto] {$\textcolor{blue}{\varepsilon_\invamp}$} (40);
  \draw (147.7bp,66.055bp) node[auto] {$$};
  \draw (390.47bp,25.977bp) node[auto] {$$};
  \draw [->,>=Implies,double equal sign distance] (31) ..controls (916.92bp,66.0bp) and (936.33bp,66.0bp)  .. node[auto] {$\textcolor{red}{\varepsilon_\otimes}$} (6);
  \draw (909.21bp,60.0bp) node[auto] {$$};
  \draw (955.89bp,60.0bp) node[auto] {$$};
  \draw [->,tips=false,double equal sign distance] (40) ..controls (471.19bp,18.402bp) and (569.67bp,0.0000bp)  .. (653.0bp,0.0bp) .. controls (653.0bp,0.0bp) and (653.0bp,0.0bp)  .. (886.0bp,0.0bp) .. controls (916.51bp,0.0bp) and (943.76bp,24.43bp)  .. node[auto] {$$} (6);
  \draw [->,>=Implies,double equal sign distance] (40) ..controls (503.18bp,36.737bp) and (769.69bp,57.216bp)  .. node[auto] {$\textcolor{red}{\eta_\otimes}$} (31);
  \draw (438.73bp,25.324bp) node[auto] {$$};
  \draw (860.61bp,58.664bp) node[auto] {$$};
%
